FullPack: Full Vector Utilization for Sub-Byte Quantized Inference on General Purpose CPUs

Although prior art has demonstrated negligible accuracy drop in sub-byte quantization -- where weights and/or activations are represented by less than 8 bits -- popular SIMD instructions of CPUs do not natively support these datatypes. While recent methods, such as ULPPACK, are already using sub-byte quantization on general-purpose CPUs with vector units, they leave out several empty bits between the sub-byte values in memory and in vector registers to avoid overflow to the neighbours during the operations. This results in memory footprint and bandwidth-usage inefficiencies and suboptimal performance. In this paper, we present memory layouts for storing, and mechanisms for processing sub-byte (4-, 2-, or 1-bit) models that utilize all the bits in the memory as well as in the vector registers for the actual data. We provide compute kernels for the proposed layout for the GEMV (GEneral Matrix-Vector multiplication) operations between weights and activations of different datatypes (e.g., 8-bit activations and 4-bit weights). For evaluation, we extended the TFLite package and added our methods to it, then ran the models on the cycle-accurate gem5 simulator to compare detailed memory and CPU cycles of each method. We compare against nine other methods that are actively used in production including GEMLOWP, Ruy, XNNPack, and ULPPACK. Furthermore, we explore the effect of different input and output sizes of deep learning layers on the performance of our proposed method. Experimental results show 0.96-2.1x speedup for small sizes and 1.2-6.7x speedup for mid to large sizes. Applying our proposal to a real-world speech recognition model, Mozilla DeepSpeech, we proved that our method achieves 1.56-2.11x end-to-end speedup compared to the state-of-the-art, depending on the bit-width employed.

==> Sections/motivation.tex <==
\section{Motivation to Focus on GEMV}
\label{backgroundAndMotivation}
	

	
	Matrix Multiplication is at the heart of most of the DNNs including, CNNs, Linear Networks, RNNs, and even Transformers.
	GEneral Matrix-Vector multiplication (GEMV) is a special case where the first matrix is a vector.
	This case is particularly being used in RNNs (e.g., LSTM and GRU) and Linear Networks with a single batch of data at each inference iteration.
	Our experiments on Mozilla DeepSpeech model measured on Gem5 (Figure~\ref{fig:deepspeechLayerBreakdown}) show that the single-batch
	LSTM layer accounts for more than $60\%$ of the whole model execution time despite the fact that there are five more
	multi-batch Linear layers, including three layers with the same unit count, in the model.
	In the same figure, we can also see the considerable gap between the runtime of the quantized model vs the full precision model as 
	the former is over 1.76x faster than the latter. \goudarzi[I don't see the point in this sentence. It's obvious, yes; but why do you need to tell
	this to the reader? Do you want to motivate "quantization"? But that's not the focus of this paper. If you want to motivate W1A1 and others, then
	clearly state that one instead. I guess you want to say that by focusing on GEMV, here is the gains that one can get on a real world complex
	application as will be described and detailed later in the manuscript, right? Either way, tell it explicitly in the text.]
	
	\goudarzi[Are the results coming from Gem5? or measurement on mobile phone? Correct the above text, if needed, accordingly. I thought it's Gem5 
	because I thought you didn't measure W1A1 etc. on mobile phone (which I don't remember why), but I could be wrong because if Gem5, then I 
	wonder how you came up with the "milliseconds" on the horizontal axis instead of cycle count.]
	
	\goudarzi[Also, this section is not "Motivation" nor "Background" for the proposal you put on the table. It's mainly arguing on why GEMV 
	was chosen as the focus. So, I changed the title accordingly, unless you want to expand it and put more motivational stuff, specifically
	showing the waste of bits by ULPack.]

				
				
				
				
				
			
				



\navid[@Hossein, Are you going to expand this Section?]


